Demystifying Map Space Exploration for NPUs

Map Space Exploration is the problem of finding optimized mappings of a Deep Neural Network (DNN) model on an accelerator. It is known to be extremely computationally expensive, and there has been active research looking at both heuristics and learning-based methods to make the problem computationally tractable. However, while there are dozens of mappers out there (all empirically claiming to find better mappings than others), the research community lacks systematic insights on how different search techniques navigate the map-space and how different mapping axes contribute to the accelerator's performance and efficiency. Such insights are crucial to developing mapping frameworks for emerging DNNs that are increasingly irregular (due to neural architecture search) and sparse, making the corresponding map spaces much more complex. In this work, rather than proposing yet another mapper, we do a first-of-its-kind apples-to-apples comparison of search techniques leveraged by different mappers. Next, we extract the learnings from our study and propose two new techniques that can augment existing mappers -- warm-start and sparsity-aware -- that demonstrate speedups, scalability, and robustness across diverse DNN models.

==> figure/architecture.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/architecture.pdf}
\end{center}
\vspace{-0.40cm}
    \caption{An example abstract DNN accelerator architecture.}

\label{fig:architecture}
\end{figure}




==> figure/maestro_timeloop_cpr.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/maestro_timloop_cpr.pdf}
\end{center}
\vspace{-0.40cm}
\caption{The comparisons of Timeloop and Maestro reported latency using the same NVDLA-like mapping (\autoref{fig:nvdla_like_mapping}) on the same acceleator configuration (Accel-B) across different workloads selected from Resnet~\cite{resnet}, VGG~\cite{vgg}, and Mnasnet~\cite{mnasnet}. \TK{can be removed?}}

\label{fig:maestro_timloop_cpr}
\end{figure}




==> figure/mapper_cpr_set1.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/mapper_cpr_set1.pdf}
\end{center}
\vspace{-0.40cm}
    \caption{Mapper Comparisons on different layers.}
\vspace{-0.1cm}
\label{fig:mapper_cpr_set1}
\end{figure}




==> figure/mapper_cpr_set2.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/mapper_cpr_set2.pdf}
\end{center}
\vspace{-0.40cm}
    \caption{Mapper Comparisons on different layers.}
\vspace{-0.1cm}
\label{fig:mapper_cpr_set2}
\end{figure}




==> figure/mappers.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/mappers.pdf}
\end{center}
\vspace{-0.40cm}
\caption{Types of Mappers (searching algorithms).}

\label{fig:mappers}
\end{figure}




==> figure/multiobjective_opt.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/multiobjective_opt.pdf}
\end{center}
\vspace{-0.40cm}
\caption{Multi-objective is used through the progress of optimization. EDP is used to select the final solution. \FK{Can be removed to save space.}}

\label{fig:multiobjective_opt}
\end{figure}




==> figure/notation.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/notation.pdf}
\end{center}
\vspace{-0.40cm}
\caption{Loop-nest representation of CONV2D and GEMM and their tensor dimension notations.}

\label{fig:notation}
\end{figure}




==> figure/nvdla_like_mapping.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{Figures/nvdla_like_mapping.pdf}
\end{center}
\vspace{-0.40cm}
    \caption{Representation of a NVDLA-like~\cite{nvdla} mapping.}

\label{fig:nvdla_like_mapping}
\end{figure}




==> figure/operator_exp.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/operator_exp.pdf}
\end{center}
\vspace{-0.40cm}
\caption{The sensitivity analysis of different mapping axes using the GA-based mapper, Gamma~\cite{gamma}. Crossover/  Tile/ Order/ Parallelism: means we enable the exploration of the corresponding axis. E.g., Tile (orange): means only tile is explored, and other mapping axes are fixed. Standard-GA uses the standard mutation and crossover (without domain-specific operators along each mapping axes described above.}

\label{fig:operator_exp}
\end{figure*}




==> figure/represent_effect.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/represent_effect.pdf}
\end{center}
\vspace{-0.40cm}
\caption{Size of search space created by naive representation and the efficient representation used in this paper (under Accel-B configuration).}

\label{fig:represent_effect}
\end{figure}




==> figure/similar_check.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{Figures/similar_check.pdf}
\end{center}
\vspace{-0.40cm}
\caption{The workflow of warm-start.}

\label{fig:similar_check}
\end{figure}




==> tables/accel_config_table.tex <==
\begin{table}[t]

\centering
\caption{The evaluating accelerator configurations.}


\includegraphics[width=1\linewidth]{Figures/accel_config_table.pdf}

\label{table:accel_config_table}
\end{table}


==> tables/dw_conv_exp.tex <==

\begin{table}[t]

\centering
\caption{The performance comparisons of different workload using depth-wise separable convolution over standard convolution. DW: Depth-wise CONV. PW: Point-wise CONV. CONV: a standard 2D CONV.}


\includegraphics[width=1\linewidth]{Figures/dw_conv_exp.pdf}

\label{table:dw_conv_exp}
\end{table}


==> tables/noc_type.tex <==
\begin{table}[t]

\centering
\caption{The NoCs HW choices.}


\includegraphics[width=1\linewidth]{Figures/noc_type.pdf}
\vspace{-0.5cm}
\label{table:noc_type}
\end{table}


==> tables/related_works.tex <==
\begin{table}[t]

\centering
\caption{Efficient Transformers and their potential buffer requirement reduction via the proposed \dataflow dataflow optimization. \TK{define what N, M, K, and R is}}


\includegraphics[width=1\linewidth]{Figures/related_works.pdf}
\vspace{-0.5cm}
\label{table:related_works}
\end{table}


==> tables/s2_buffer_size.tex <==
\begin{table}[t]

\centering
\caption{The on-chip buffer size requirement to stage weights and activations on-chip. H: number of heads, N: sequence length, D: hidden dimension size.}

\vspace{-0.3cm}
\includegraphics[width=1\linewidth]{Figures/buffer_size.pdf}

\label{table:buffer_size}
\end{table}


==> tables/s3_l3_size_of_example.tex <==
\begin{table}[t]

\centering
\caption{Buffer requirement for tiling granularity. M: batched Multi-head, B: Batch, H: Head, R: Row.}

\vspace{-0.3cm}
\includegraphics[width=1\linewidth]{Figures/l3_size_of_example.pdf}
\vspace{-0.5cm}
\label{table:l3_size_of_example}
\end{table}


==> tables/s5_cloud_edge_config.tex <==
\begin{table}[t]

\centering
\caption{The HW resource configuration of cloud and edge accelerators in the evaluation sections.}


\includegraphics[width=1\linewidth]{Figures/cloud_edge_config.pdf}

\label{table:cloud_edge_config}
\end{table}


==> tables/s5_cpr_more_models.tex <==


\begin{table}[t]

\centering
\caption{The speedup ratio of \system to FlexAccel-cstr-BMH and \system to FlexAccel on different models and resources with the respect to end-to-end runtime.\TK{Convert to geo-mean. Possible waay to reduce space -- combine Table 4 and 5 into one table, with runtime and energy.}}


\includegraphics[width=1\linewidth]{Figures/cpr_more_models.pdf}

\label{table:cpr_more_models}
\end{table}


==> tables/s5_cpr_more_models_energy.tex <==


\begin{table}[t]

\centering
\caption{The energy-consumption of \system to FlexAccel-cstr-BMH and \system to FlexAccel on different models and resources with the respect to end-to-end energy consumption.\TK{convention not clear, what are the two numbers in each cell. Caption should explain}}


\includegraphics[width=1\linewidth]{Figures/cpr_more_models_energy.pdf}

\label{table:cpr_more_models_energy}
\end{table}


==> tables/warm_start_table_resnet.tex <==
\begin{table}[h]

\centering
\caption{The effect of warm-start on Resnet-18.}


\includegraphics[width=1\linewidth]{Figures/warm_start_table_resnet.pdf}

\label{table:warm_start_table_resnet}
\end{table}

